The Sands of Phobos: The Martian moon's eccentric orbit refreshes its surface

The surface of the Martian moon Phobos exhibits two distinct geologic units, known as the red and blue units. The provenance of these regions is uncertain yet crucial to understanding the origin of the Martian moon and its interaction with the space environment. Here we show that Phobos' orbital eccentricity can cause sufficient grain motion to refresh its surface, suggesting that space weathering is the likely driver of the dichotomy on the moon's surface. In particular, we predict that blue regions are made up of pristine endogenic material that can be uncovered in steep terrain subject to large variations in the tidal forcing from Mars. The predictions of our model are consistent with current spacecraft observations which show that blue units are found near these regions.

==> tables.tex <==
\section*{Tables}

\begin{table}[h]
\centering
\begin{tabular}{l l l}
\hline
\textbf{Property} & \textbf{Low Resolution} & \textbf{High Resolution}\\
\hline
$R_{\mathrm{grain}}$ & 1.4-1.6 cm & 0.09-0.11 cm \\
$\phi$ & 32$^{\circ}$ & 32$^{\circ}$ \\
$\rho_{\mathrm{grain}}$ & 3.1 g cm$^{-3}$ & 3.1 g cm$^{-3}$ \\
$\rho_{\mathrm{bulk}}$ & 1.7 g cm$^{-3}$ & 1.7 g cm$^{-3}$ \\
$N$ & 7,000 & 50,000 \\
Sim. Area & 1.5 $\times$ 1.2 m & 0.60 $\times$ 0.4 m \\
\hline
\end{tabular}
\caption{Properties of simulated regolith for granular dynamics simulations. $R_{\mathrm{grain}}$: grain radius, $\phi$: critical angle, $\rho_{\mathrm{grain}}$: grain density, $\rho_{\mathrm{bulk}}$: grain bed bulk density, $N$: number of particles, Sim. Area: surface area of grain bed.  }
\end{table}

